Fragmented Objects: Boosting Concurrency of Shared Large Objects

This work examines strategies to handle large shared data objects in distributed storage systems (DSS), while boosting the number of concurrent accesses, maintaining strong consistency guarantees, and ensuring good operation performance. To this respect, we define the notion of fragmented objects:con-current objects composed of a list of fragments (or blocks) that allow operations to manipulate each of their fragments individually. As the fragments belong to the same object, it is not enough that each fragment is linearizable to have useful consistency guarantees in the composed object. Hence, we capture the consistency semantic of the whole object with the notion of fragmented linearizability. Then, considering that a variance of linearizability, coverability, is more suited for versioned objects like files, we provide an implementation of a distributed file system, called COBFS, that utilizes coverable fragmented objects (i.e., files).In COBFS, each file is a linked-list of coverable block objects. Preliminary emulation of COBFS demonstrates the potential of our approach in boosting the concurrency of strongly consistent large objects.

==> architcture_v1.tex <==
\section{System Architecture}


==> emulation_v1.tex <==
\section{Prototype Implementation}
\label{sec:implementation}

Having laid out the theoretical basis of Fragmented Objects with Coverable Blocks, we now present a case study to demonstrate how the algorithm can be leveraged in a Distributed File System to handle large objects. In our prototype implementation we consider each object to be a plain text file, however the underlying theoretical formulation allows for extending this implementation to support any kind of large objects.

\begin{figure}[h]
\centering
\subfloat{\includegraphics[width=0.9\linewidth]{File_Fragmentation/architecture/architecture.png}}
\caption{Basic architecture}
\label{fig:architecture}
\end{figure}

%An overview on how we use the {\em rolling hashing} technique to break files into blocks and implement the files as fragmented objects satisfying {\em fragmented linearizability}.

\textbf{Basic Architecure:} Access for clients to the file system is granted through reader/writer processes, while the blocks of each file are maintained by servers.  The core concept of our implementation is the Fragmentation Module (FM). Each client has a FM responsible for fragmenting the file into blocks and having each block updated on the servers. The implementation of the FM is based on the RSYNC (Remote Sync) algorithm ~\cite{rsync}. 
RSYNC identifies and transfers only \st{parts} \thc{chunks} of a file at the client that either 
(i) do not exist on servers 
or 
(ii) they have been modified. 
% 
% Block boundaries are identified according to a rolling hash algorithm. 
The implementation of rolling hash that we use, is the {\em rabin fingerprints}~\cite{rabin}. It identifies the block boundaries and it performs content-based chunking by
calculating the fingerprints over a sliding window. This strategy is defined at the client level, as shown in Fig.~\ref{fig:architecture}. 

\textbf{Maintaining Blocks in Practice:}
In this prototype implementation identifying changes in a fragmented object and dividing data into appropriately sized blocks (e.g., when updating or writing new values), are performed as follows:

\begin{itemize}[leftmargin=10mm]
  \item Initially, the \emph{FM} partitions a file into blocks based on its contents, using \emph{rabin fingerprints}. This algorithm guarantees that when a file is changed, 
  \thc{in the worst case,}
  only the hash of a modified block and its next one are affected, 
    %   and in the worst case its next one) 
    % is affected, 
  but not those of subsequent blocks. 
  
  \item Next, the \emph{FM} compares the sequence of the hashes computed in the first step \thc{with} the sequence of hashes of the currently managed blocks. 
  The comparison yields the list of hashes that have been 
  (i) replaced, 
  (ii) inserted, 
  (iii) deleted and, 
  (iv) remained unchanged. 
  In the case (i) of replacement, the block id $b_{id}$ is preserved, while the old hash is replaced with the new hash. In the case (ii) of insertion, a new $b_{id}$ has to be created and associated to the new hash. In the case (iii) of deleting, the block id $b_{id}$ is remained the same and associated to a zero hash value, i.e. an empty file. Lastly, in the case (iv) of equality, the $b_{id}$ remains the same. As a result, a sequence of $b_{ids}$ associated with its hashes is created. 
 
  \item Lastly, modified and newly created blocks are transmitted to the replica servers. 
\end{itemize}

For example, the schematic in Fig.~\ref{fig:example} shows a writer process with id $x$ writing new text at the beginning of the second block of a text file with id $f_{id}=7$. Notice, how the hash value of the existing second block ``$4bad..$'' is replaced with ``$d595..$'' and a new block with hash value ``$8223..$'' is inserted immediately after, extending the second block. 
% A new block with $b_{id} = $ x{\_}7-x{\_}4 is assigned. 
Lastly, the modified block with $b_{id} = $ x{\_}7-x{\_}2
and the new block with $b_{id} = $ x{\_}7-x{\_}4 are sent to the replica servers.

\begin{figure}[t]
\centering
\subfloat{\includegraphics[width=0.9\linewidth]{File_Fragmentation/architecture/fm_manager.png}}
\caption{An example of text insertion which changes the block structure... \thc{elaborate a bit more.}}
%{\bf If we need space, we can move this figure to an Appendix.}}
\label{fig:example}
\end{figure}

\textbf{Other operations:}
Besides updating the contents of a file and managing blocks, the {\em FM} supports a number of other useful operations, such as reading a file, creating a file, renaming a file, deleting a file, obtaining a list of the existing files and an advanced list operation. 
\newline
% Firstly, we must mention some structures that are used in our implementation, which will help us to describe the above operations. 
% 
\thc{
To store information about the files that the \emph{FM} manages, internally the \emph{FM} maintains a dictionary $D$. More in detail, a key entry is a file path $f_{path}$ of $f_{id}$, and the corresponding value is a tuple consisting the $b_{id}$ of the genesis block $b_{gen}$ of $f_{id}$ and  the file id $f_{id}$ of the fragmented file $f$. That is, $D: \{ key,value \} = \{ f_{path} , \langle b_{gen}, f_{id}   \rangle \}$.
}
The \emph{FM} uses $f_{path}$ as key for this dictionary, in order to be able to monitor the changes that take place for each file. However, in the level of the Atomic Shared Object Algorithm, all the information about a file is stored based on its $f_{id}$. 

It is worth mentioning that, the format of a block that sending to the Atomic Shared Object Algorithm, is a text file containing the header and the literal data of the block. The header includes some information about the block, i.e. the hash value, a boolean value that indicates if the block is the genesis one, the next $b_{id}$, the block size and the modification time of the block. If the block is the genesis block, the header it also contains the $f_{path}$. 
\newline

\begin{itemize}[leftmargin=10mm]

\item {\bf Read Operation}: In order to read a file, the \emph{FM} issues a series of block read operations; starting from the local genesis block of $f$ and proceeding to the last block by following the next $b_{id}$ that is included in the header of each block derived from the serves.  

\item {\bf Create Operation}: When a new file is created on the client's filesystem, 
the \emph{FM} 
fragments it into its respective blocks (including the genesis block), and writes them on the servers by invoking a sequence of write operations for the entirety of the blocks comprising the file. 

\item {\bf Rename Operation}: When a file is renamed on the client, the \emph{FM} executes a special write request, where it writes the genesis block of the file that includes the new $f_{path}$ in its header. 

\item {\bf Delete Operation}: When a file is deleted on the client, the \emph{FM} discards the $f_{id}$ entry from its dictionary and sends a special write request to the servers, in order to delete it as well. As a result, no further operations can be performed on the deleted file, since the \emph{FM} and the servers do not have access to its genesis block. 

\item {\bf List Operation}: To obtain the list of existing files, the {\em FM} contacts the servers and obtains the $f_{id}$, the $f_{path}$ and the genesis block id $b_{gen}$ of each file, which then allows for further read operations to be issued.

\item {\bf Advanced List Operation}: The advanced list operation, is similar to the simple list one, giving some additional information about each file. At first, the \emph{FM} requests a simple list request. Then for each file in the resulted list, it requests a series of block list operations. Each block list operation informs the \emph{FM} about the size and the modified size of the block. As a result, the \emph{FM} can calculate the size of the whole file and the maximum modified time that a block of the file has changed. 

\end{itemize}

==> fragmentation_v1.tex <==
\section{Implementing Fragmented Objects}
\label{sec:fragment}
Informally, a fragmented object is a concurrent object which maintains a sequence of fragments or blocks. We first formally define the notion of a block and then we proceed to formally define the fragmented object. 

\paragraph{Fragment/Block object.}

A \emph{fragment} or \emph{block} is a linearizable read/write concurrent object with a unique identifier from a set  $\blockSet\subset\fileSet\times\cSet\times\Nat$,
where $\fileSet$ is the set of fragmented objects identifiers. In particular, the identifier of a block $b\in \blockSet$ is the triple $\tup{fid, cid, cseq}$, where $fid\in\fileSet$ is the identifier of the fragmented object in which the block belongs to, $cid\in\cSet$ is the identifier of the process that created the block, %(as we will see below this is not necessarily the owner/creator of the file), 
and $cseq\in\Nat$ is the process' local sequence number that it is incremented every time this process creates a block for this fragmented object (this ensures the uniqueness of 
the blocks created by the same client for the same fragmented object).\vspace{.5em}
 
Each block $b \in\blockSet$ is associated with two structures, $val$ and $ver$.
\begin{itemize}[leftmargin=3mm]
\item $val(b)$ is composed of: (i) a \emph{pointer} that points to the next block ($\bot$ denotes the null pointer), and (ii) the \emph{data} contained in the block ($\bot$ means there are no data).   
\item $ver(b)=\tup{wid,bseq}$, where $wid\in\cSet$ is the
identifier of the client that last updated $val(b)$ (initially is the id of the creator of the block) and
$bseq\in\Nat$ is a sequence number of the block (initially 0) that it is incremented every time $val(b)$ is updated. 
\end{itemize}

In other words, $val(b)$ represents the content of the block along with its ``position'' in the fragmented object and $ver(b)$ is used for ordering the update operations performed on the block (these operations are detail below). We will be using the ``.'' operand to refer to the components of $val()$ and $ver()$; e.g., $val(b).data$ denotes the data of block $b$.\vspace{.5em}  
 

 
%The block can be simply the identifier of the next %fragment or used as in IPFS \cite{} and hold some 
%extra information to enhance security of the service. 
%that is composed of three fields takes values from a set $\valSet$,
We assume that each block $b$ can have a maximum {\em fixed} size $\ell$ (measured in MBs), i.e.,  $|value(b).data|\leq \ell$.
Depending on the application, $\ell$ could have a different value. For example, in GFS $\ell=64$MB whereas in Colossus (successor of GFS) 
$\ell=1$MB. 
%[[An empirical study could identify interesting tradeoffs between 
%$\ell$ and operation latency and overall system performance.]]
\vspace{.5em}

\sloppy{Given a block $b$ and $ver_1(b), ver_2(b)$ we define the order $<_{v}$  as follows: 
$ver_1(b) <_{v} ver_2(b)$ \textbf{iff} $ver_1(b).bseq<ver_2(b).bseq$ \textbf{or} $(ver_1(b).bseq == ver_2(b).bseq$ \textbf{and} 
$ver_1(b).wid < ver_2(b).wid)$.}\vspace{.5em}  


\noindent Operations on block $b$ by processor $p$ (all operations are atomic): 
\begin{itemize}[leftmargin=3mm]
    \item $\act{create}(\tup{fid,p,cseq_p},\tup{ptr,D},\tup{p,0})$: Processor $p$ creates block $b=\tup{fid,p,cseq_p}$ for  $fid$ with $val(b).data=D, val(b).pointer=ptr, ver(b).wid=p$ and $ver(b).bseq=0$. It returns \texttt{OK}. 
	\item $\act{read}()_b$: It reads the state of block $b$; i.e., it returns $(val(b),ver(b))$.
	\item $\act{write}(\tup{ptr,D},\tup{p,seq})_b$: \sloppy{It attempts to modify the state of block $b$;} it returns \texttt{success} or $(val(b),ver(b))$ if $\tup{p,seq} <_{v} ver(b)$.
\end{itemize}	


Observe that we have not defined a ``delete" operation on blocks. The contents of a block can be erased (by issuing a write with $D=\bot$) but for technical reasons we explain below, we do not wish for blocks to be removed. We now proceed to define a fragmented object as a sequence (linked-list) of blocks.\vspace{.5em}





%%%%%%%%%%%%%%%%%% removing old block ops
\remove{ %%%% remove start

%\noindent {\bf [[Once we agree we will update them to %coverable objects]]}\\
\noindent Operations on block $b$ (all operations are atomic): 
\begin{itemize}
	\item $\act{read}()_b$: It reads block $b$; i.e., it returns $(val(b),ver(b))$.
	\item $\act{write}(val(b),ver(b))_b$: \sloppy{It attempts to modify the block; it returns \texttt{success} or $(val(b),ver(b))$.} If $b$ is a new block, then this operation, performed say by client $p$, essentially creates $b$, in which case $b=\tup{fid,p,cseq_p}$, $val(b).pointer$ will need to be specified (see the next operation below) and $(ver(b).wid=p,ver(b).bseq=0)$.
	Once a block is created, its content can be erased (by writing  $val(b).data=\bot$), but it cannot be removed, that is, $val(b).pointer$ cannot be changed to $\bot$ or have no other block pointing at it (unless the whole file is deleted -- see below). We do not remove blocks, as concurrent writes on neighboring blocks could easily break the continuity of block chains. 
	\item $\act{extend}((val(b).pointer=b_1,val(b).data),ver(b)),\tup{b_1,\ldots,b_x})_b$: It attempts to extend $b$; it returns \texttt{success} or $(val(b),ver(b))$. O Its content canIf the $\act{write}$ operation writes, then this means that the block is  
	This operation can only be triggered in the case that an update on the data of $b$ forces the size of $b$ to exceed $\ell$. 
	This operation, if successful, creates the blocks 
	$b_1,\ldots,b_x$ (as explained above) with pointers such that $\tup{b_1,\ldots,b_x}$ is a block chain that extends $b$ as defined above).\footnote{This is essentially the atomic execution of the following operations: $\act{write}((val(b_1).pointer=b_2,val(b_1).data),(ver(b_1).wid=p,ver(b_1).bseq=0)_b{_1},\act{write}((val(b_2).pointer=b_3,val(b_2).data),(ver(b_2).wid=p,ver(b_2).bseq=0)_b{_2},\ldots,\act{write}((val(b_x).pointer=b',val(b_x).data),(ver(b_x).wid=p,ver(b_x).bseq=0)_b{_x}$ and $\act{write}((val(b).pointer=b_1,val(b).data),(ver(b).wid=p,ver(b).bseq)_b$; $p$ is the client performing  $\act{extend}$ and $b'$ is the block that $b$ pointed at before the extend operation.}
	%\item $\act{erase}()_b$: It empties the data of the block \underline{without} nullifying its pointer. I.e., it calls 
	%$\act{write(val(b),ver(b)) that returns $b.data = \bot$. ()  
\end{itemize}

Creating a new block is only allowed within the extend operation (which will call the write operation for a new block). Furthermore, no two or more blocks can point to the same block. We need an one to one and onto relation between blocks in any block chain. [[Perhaps it is best to create a create operation (which will essentially be a write operation as described above) and say that this operation can only be called by the extend operation -- this should make things more clear. Also, extend is the only operation that can change the pointer of a block.]] \vspace{.5em}
} % END remove
%%%%%%%%%%%%%%%% REMOVE %%%%%


We will be referring to a {\em block linked-list} as a continuous linked list
of blocks of the same fragmented object. For example, $\tup{b_1,b_2,b_3,b_4}$ is a block linked-list if and only if $val(b_1).pointer = b_2,~val(b_2).pointer = b_3,$ and $val(b_3).pointer = b_4$ and $b_1.fid=b_2.fid=b_3.fid=b_4.fid$. 

Let {\em fnode} be a read only block pointer, unique for each fragmented object. Then a block linked-list is {\em complete} iff the $fnode$ points to the first block of the chain, and the last block (which could be the first and only block) points to $\bot$.  
\vspace{.5em}

\paragraph{Fragmented object.}
A \emph{fragmented object}  is a complete block linked-list with a unique identifier from a set  
$\fileSet\subseteq\cSet\times\Nat$. In particular, the identifier of the object $f\in\fileSet$ is a pair $\tup{cfid,cfseq}$, where $cfid\in\cSet$ is the identifier of the client that created the fragmented object and $cfseq\in\Nat$ is the client's local sequence number that it is incremented every time this client creates a fragmented object (this ensures the uniqueness of the objects created by the same client). %Each file uses a read only \emph{bnode} that points to the first block of the list.
In other words, a fragmented object $f$ is a linked-list of blocks  $\langle b_1,\ldots, b_q\rangle$ if and only if
$fnode=b_1$ and $val(b_q).pointer = \bot$; $q\geq 1$ is a variable that can only monotonically increase and represents the \emph{object size} of the object wrt number of blocks. To be more precise, each fragmented object id $f$ is associated with its linked-list of blocks. Each fragmented object id is also associated with a boolean $active$, which initially is true; when this is turned to false, its marks that the object is deleted (no further operations can be performed).\vspace{.5em}

For the modify operation detailed below, the following definition is needed: Consider a block $b$ that points to $b'\in \blockSet\cup\{\bot\}$. We say that the block linked-list $\tup{b_1,\ldots, b_x}$, $x\geq 1$, \emph{extends} block $b$, if and only if $val(b).pointer = b_1$ and $val(b_x).pointer = b'$.\vspace{.5em}  

\noindent  Operations on object $f$ by processor $p$: %(all operations are atomic):
\begin{itemize}[leftmargin=3mm]
	%\item $\act{insert}(i, j)$: insert fragment with identifier $i\in%\blockSet$ after fragment $j\in\blockSet$
	\item $\act{create}(\tup{p,cfseq_p},fnode)$: Processor $p$ creates the fragmented object with id $f=\tup{p,cseq_p}$ initialized to the sequence $\tup{b=\tup{f,p,cseq_p}}$ where $fnode=b$ and $val(b).pointer = \bot$\footnote{In an atomic step it calls $\act{create}(\tup{f,p,cseq_p},\tup{\bot,D},\tup{p,0})$ and sets $fnode=\tup{f,p,cseq_p}$ and $f.active=true$.}. It returns \texttt{OK}. In other words, it creates the first block of the object, which we call {\em the genesis block} of the fragmented object.  
	\item $\act{retrieve}()_f$:  retrieves the whole object, starting from the genesis block and reaching the last block (with a pointer to $\bot$). Ie, it returns the sequence: $\tup{b_1,\ldots,b_q}$, where $fnode=b_1,val(b_q).pointer=\bot,$ and $q$ is the size of the object\footnote{It calls $\act{read}()_{b_i}$ for all blocks $b_i$ in the linked-list (from the one $fnode$ points to -- genesis block-- until the one pointing to $\bot$).}. 
	\item $\act{modify}()_f$: attempts to write the blocks that $p$ has changed and extends the ones that exceed the block size $\ell$. In particular, consider the following two cases regarding each block $b$ that $p$ has changed (and the modify operation will attempt to write). Let $D=val(b).data$ be the data content after $p$ updates. Then: 
	\begin{itemize}
	\item $\mathbf{|D|\leq \ell}$: In this case $\act{modify}$, for block $b$, calls  $\act{write}(\tup{val(b).pointer,D},\tup{p,bseq\mathrm{++}})_b$.     
	\item $\mathbf{|D|> \ell}$: In this case, the data needs to be broken into chunks of size $\ell$ (except possibly the last one). Say that $D$ is broken into $x$ chunks, $D_0$ to $D_{x-1}$. The corresponding sequence $(\tup{b_1,\ldots,b_{x-1}})$ is created to extend $b$; assume that currently $val(b).pointer=b'$. Then, the following block operations are performed in this particular order: \sloppy{$\act{create}(b_{x-1}=\tup{f,p,cseq_p\mathrm{++}},\tup{b',D_{x-1}},\tup{p,0}),\ldots,\act{create}(b_1=\tup{f,p,cseq_p\mathrm{++}},\tup{b_2,D_1},\tup{p,0})$ and $\act{write}(\tup{b_1,D_0},\tup{p,bseq\mathrm{++}})_b$.} Observe that all these are done atomically since it involves the creation of blocks with unique ids. If the last write does not succeed, then the whole extension essentially does not succeed. 
	\end{itemize}
	 
	\item $\act{delete}()_f$: It deletes object $f$; it sets $f.active=false$ and returns \texttt{OK}. It is understood that all block and object operations are valid as long as the certain object is active. (The fragmented object id is not reused.) 
	%\item $\act{save}()$:  writes all the fragments that changed and inserts new fragments
	 %\item $\act{read}(f_i)$: retrieves the value of the fragment $f_i\in\blockSet$ 
	 %\item $\act{write}(val, f_i)$: replace the value of the fragment $f_i\in\blockSet$ with val. first fragment 
\end{itemize} 


%WE NEED TO ENSURE THAT THE FILE OPERATIONS (ESSENTIALLY MODIFY) MAINTAIN A COMPLETE BLOCK CHAIN. (From the description of modify it is not difficult to see that this is the case -- no matter if the update succeeds of not.)

%Note that we assume that we do not perform remove operations on the list. We assume that
%fragments may become empty. \nn{Maybe we should think about remove or introduce a garbage collection mechanism.} 
